Preferential Mixture-of-Experts: Interpretable Models that Rely on Human Expertise as much as Possible

We propose Preferential MoE, a novel human-ML mixture-of-experts model that augments human expertise in decision making with a data-based classifier only when necessary for predictive performance. Our model exhibits an interpretable gating function that provides information on when human rules should be followed or avoided. The gating function is maximized for using human-based rules, and classification errors are minimized. We propose solving a coupled multi-objective problem with convex subproblems. We develop approximate algorithms and study their performance and convergence. Finally, we demonstrate the utility of Preferential MoE on two clinical applications for the treatment of Human Immunodeficiency Virus (HIV) and management of Major Depressive Disorder (MDD).

==> 01_intro.tex <==
\section{Introduction}

\begin{itemize}
	\item When facing a prediction task, clinicians often rely on guidelines/rules of thumb/heuristics that reflect common clinical practice.
	\item Recently, ML-advise human decision making systems proposed: ML systems used in conjunction with human guidelines.
	**\item Advantages of following human guidelines (see below)
	**\item But how good are these guidelines?
	**\item When ML system in disagreement with human guidelines, tension  arises (example of excitatory med recommended by AI: maybe there exists any equivalent drug that does the same without negative drawbacks). Does the ML system disagrees because the guideline is wrong, or because there is an alternative recommendation that would also work?
	\item Ideally, we would like to disagree with human guidelines \emph{only} when needed (as little as necessary), complementary strengths of humans and ML-systems. 
	\item We develop a ML system that incorporates human expertise, and aligns with human guidelines as much as possible without performance loss. The proposed approach can advise whether to follow or not the guidelines, and give an alternative data-based prediction.
	\item Contribution: Interpretable Mixture of Experts where one expert is a human (data-based model as a residual). Goal is to follow expert rules as much as possible: MoE with preference for one expert (human) whenever possible. Useful to identify when we should follow human vs when we should follow data-based classifier (interpretable gating function).
	\item We give a solution to how to enforce preference for human expert + how to get interpretable gating function
\end{itemize}

% MEL: maybe dangerous argument but I let it here just in case
%One of the reasons why ML systems are not widely spread in the clinic is because these do not incorporate expert knowledge from clinicians, intuitions, additional information that might not be captured by a data-driven approach.

Advantages of following the rules.

\begin{itemize}
	\item Credibility: a model that aligns with human knowledge when possible is easier to trust, inspect, and more useful/likely to deploy (citation Credible models). Detect input-regions where rules can be followed (trust).
	
	\item Extrinsic motivation: benefits not captured by accuracy: safety, tolerability, cost, etc (e.g., do not recommend a violent movie to a minor; do not give excitatory meds to a person that has insomnia).
	
	\item Predictive preformance: eventually, rules might help improve accuracy (if guidelines aligned with outcome).
	
	\item Humans remain in charge
	\begin{itemize}
		\item current status-quo, so interventions that suggest minimal (differential) changes will be easier to deploy
		\item Humans do not loose faculties or cognitive engagement
	\end{itemize}
	
\end{itemize}

\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{figs/desiderata}
	\caption{Complementary ML-system: only disagrees with human guidelines when these are inadequate; our approach also provides additional information (types of uncertainty w.r.t the rule)}
	\label{fig:desiderata}
\end{figure}

==> 02_related_work.tex <==
\section{Related work}

%	% MEL: should we talk about logic-based or posterior regularization?
%\paragraph{Other approaches to incorporate human expertise}  (MEL: Confirm relevance first, then complete)
%\begin{enumerate}
%	\item \textbf{Constrained optimization}: (Lorenzi et.al, 2017; Ross et.al, 2019)
%	\begin{itemize}
%		\item \textbf{Credible models}. Human expertise at the input-level (Wang et.al, 2019)
%	\end{itemize}
%	%\item \textbf{Logic-based approaches} (like Probabilistic Soft Logic - Bach et.al, 2017)
%	%\item \textbf{Posterior regularization}: (Gollapalli, Li, and Yang 2017; Xu et al. 2017; Tavares et.al, 2019): e.g., semantic loss, logic + probabilities computed by network
%\end{enumerate}

\begin{itemize}
	\item Human-AI decision making systems based on mixture of experts:
	\begin{itemize}
		\item Learn to defer
		\item Experts that chooses to accept/reject decision of classifier (Bansal et.al, 2019, 2020)
	\end{itemize}
	\item Other ways to incorporate human expertise
	\begin{itemize}
		\item Credible models (Wang et.al, 2019)
		\item Knowledge distillation
		\item Architecture modification
		\item Posterior regularization
	\end{itemize}
\end{itemize}

\subsection{Human-AI decision making systems based on mixture of experts}

\paragraph{Learning to defer approaches.}
Models as triage tools, when querying humans is a limited resource, so most observations
are handled automatically by the data-driven classifier, and only
a few (most difficult) observations are deferred to human experts (citation X-ray paper). Different goal: Human decisions, but expensive to query (most often, use ML and rely on humans as little as possible, only for the hard examples)
In our case, humans take the lead. It is the complementary: rely on humans as much as possible except for those regions for which human guidelines are wrong
Different human input: Train classifier based on human decisions as labels
Instead, we assume the presence of some (partial, generic) rules specified by humans.

\begin{itemize}
	\item (Mozannar et.al, 2020) Consistent Estimators for Learning to Defer
	to an Expert: propose a MoE that can either predict or defer to a
	human. Same framework as (Madras et.al, 2018), but does not allow
	the model to adapt to the underlying human expert (??)
	\begin{itemize}
		\item approaches for ML models that can predict or defer the decision to
		a downstream expert (complementary)
		\item learned model adapts to human expert, model focuses on regions there
		expert is less accurate
		\item 0-1 missclasification error
		\item cost sensitive learning problem over augmented label space that includes
		action of deferral
	\end{itemize}
	\item (Madras et.al, 2018) Predict responsibly: Improving fairness and accuracy
	by learning to defer
	\begin{itemize}
		\item model does not adapt to underlying expert (trained in all space?)
		\item loss not consistent
		\item requires uncertainty estimate of the expert decisions
	\end{itemize}
	\item (Raghu et.al, 2019) The algorithmic automation problem: Prediction,
	triage, and human effort.
	\begin{itemize}
		\item learns classifier for all data ignoring expert, then obtains uncertainty
		estimates for both the expert and data-based classifier, and defer
		based on which is higher.
	\end{itemize}
	\item (Wilder et.al, 2020) Learning to complement humans
	\begin{itemize}
		\item Similar tp (Raghu et.al, 2019), but defers based on ML/human confidences. 
	\end{itemize}
	\item Shazeer, N., Mirhoseini, A., Maziarz, K., Davis, A., Le, Q., Hinton,
	G., and Dean, J. Outrageously large neural networks: The sparsely-gated
	mixture-of-experts layer.
	\item Hierarchical mixtures of experts and the EM algorithm. (Jordan and
	Jacobs, 1994): origin of MoE type of models.
	\begin{itemize}
		\item Hard mixture of experts
	\end{itemize}
\end{itemize}

\subsection{Other ways to incorporate human expertise}

\begin{enumerate}
	\item “All symbolics” approach (like Probabilistic Soft Logic - Bach et.al, 2017)
	\item Distillation approaches: (Hu et.al, 2016), works worse if expert intuition is unreliable/random (since it is considered as ground truth through the pseudo-observations)
	\item Posterior regularization: (Gollapalli, Li, and Yang 2017; Xu et al. 2017; Tavares et.al, 2019): e.g., semantic loss, logic + probabilities computed by network
	\item Constrained optimization: (Lorenzi et.al, 2017; Ross et.al, 2019)
	\item Methods that map rules to elements of neural network: (Towell and Shavlik 1994),  (Tran and Garcez 2018).
	\begin{itemize}
		\item Fancier architectures (e.g., knowledge gates in RNNs: (Wu et al. AAAI 2016) for question answering/text matching).
	\end{itemize}
	\item Residual models: given an expert system, i.e., use data to model residual from expert system (Chatta et.al, 2019)
	\item Weakly supervised approaches
\end{enumerate}

==> 03_approach.tex <==
\section{Methodology}


In this section, we propose a ML model that complements human decision rules with data-based evidence in the training. The proposes approach should fulfill two desiderata. First, we want to rely on the human rules as much as possible while making sure the overall predictive performance is not damaged. Second, the proposed model should be interpretable, and provide additional information on how adequate (w.r.t the predictive task) each human guideline is overall, and for which patients in particular we can rely on the human guideline.

\begin{enumerate}
	\item Get a more interpretable model (extract additional information).
	\begin{itemize}
		\item Local: For which patients should we follow the human rules?
		
		\item Global: Can we detect when expert rules are wrong? Which human rules are most helpful with respect to the prediction task?
	\end{itemize}
\end{enumerate}

If the human guidelines are very damaging w.r.t the prediction task, our approach is able to overrule them (that is, we recover the same solution as the unconstrained problem).

We assume that we have access to some human guidelines. If that is not available, but instead we have samples of the experts decisions, we can train a classifier that mimics the human decisions beforehand, and use it as our human-based rule $g(x)$.

\paragraph{Objective.} We seek to constraint data-driven models with expert knowledge. In particular, given a function $f_\theta: x \mapsto y$ and a set of $K$ implication rules $(A_k \Rightarrow B_k)$, where $A_k$ and $B_k$ are the antecedent and consequent respectively, we seek to improve the agreement of $f_\theta$ with such rules, which will eventually lead to better performance/generalization of $f_\theta$.
%% MFP: Increase tolerability of treatment

\begin{itemize}
	\item Given some data $\{(x_i,y_i)\}^N_{i=1}$, we might be able to find several classifiers/regressors that have similar performance, but are qualitatively different, and thus, might generalize differently. We want to use the intuition of experts (via expert rules) to guide the optimization such that we are able to choose models that have both, high accuracy and are in stronger agreement with the expert rules.
	\item Expert rules are static, data-driven approaches might capture new insights from data. Expert rules might be incomplete, there is no clear answer once input feature is missing (else clause is very broad).
	\item \textbf{Ultimate goal}: an ML prediction system augmented with expert rules that takes into account both data evidence and expert’s intuition at prescribing  (ultimately, evaluation based on fidelity criteria to the data).
	\item In a way, we propose to add additional input features (concepts) that experts find relevant to make prescriptions, and learn the importance of such rules in the prediction.
	\item One important baseline: logistic regression with input features, conditions (antecedents), treatments (consequents), and rule compliances as inputs.
\end{itemize}

\paragraph{Predictive model} Describe mixture of experts setting. (maybe formulate more generally for Categorical distribution instead of Bernoulli)

\begin{equation}
\hat{y}_{\theta,\rho_{w}}(x)=\left\{ \begin{array}{cc}
(1-\rho_{w}(x))f_{\theta}(x)+\rho_{w}(x)g(x) & \quad\text{{if}\;}g(x)\neq-1\\
f_{\theta}(x) & \quad\text{{if}\;}g(x)=-1
\end{array}\right.\label{eq:MoE}
\end{equation}

\begin{itemize}
	\item human rule $g:\mathbb{R}^{d}\rightarrow\left\{ 1,0,-1\right\} $ 
	\item ML classifier $f_{\theta}(x):\mathbb{R}^{d}\rightarrow[0,1]$
	\item gating function $\rho_{w}:\mathbb{R}^{d}\rightarrow[0,1]$
\end{itemize}

\[
y|x\sim\mathrm{Bernoulli\,}\Big(\hat{y}_{\theta,\rho_{w}}(x)\Big)
\]

\[
y|x\sim\left\{ \begin{array}{cc}
\mathrm{Bernoulli}\Big(\big(1-\rho_{w}(x)\big)f_{\theta}(x)+\rho_{w}(x)g(x)\Big), & \mathrm{if}\,g(x)\in\{0,1\}\\
\mathrm{Bernoulli}\Big(f_{\theta}(x)\Big), & \mathrm{if}\,g(x)=-1
\end{array}\right.
\]

where $\rho_{w}(x)\in[0,1]$, $g(x)\in\{0,1,-1\}$, and $f_{\theta}(x)\in[0,1]$.

\subsection*{Problem Formulation and inference}

\begin{itemize}
	\item Performance metric, e.g, $\mathrm{BCE}(y,\hat{y})$
\end{itemize}
\begin{equation}
L_{\theta,\rho_{w}}^{\text{data}}({\cal D})=\sum_{n=1}^{N}-\left[y_{n}\ln(\hat{y}_{\theta,\rho_{w}}(x_{n}))+(1-y_{n})\ln(1-\hat{y}_{\theta,\rho_{w}}(x_{n}))\right].\label{eq:bce}
\end{equation}

\begin{itemize}
	\item Rule compliance (how often do we rely on humans?)
\end{itemize}
\begin{align}
	\max_{\theta,\rho_{w}} & \quad\rho_{w}(x)\label{eq:multi-objective-2}\\
	\text{s.t.} & \quad L_{\theta,\rho_{w}}^{\text{data}}({\cal D})\leq L_{\theta^{*},\rho_{w}^{*}}^{\text{data}}({\cal D})(1+\varepsilon)
\end{align}


Barrier function form:

\[
\min_{\theta,\rho_{w}\geq0}I_{t}(\theta,\rho;\epsilon,\mathcal{D})=\min_{\theta,\rho_{w}\geq0}\quad-t\sum_{x\in\mathcal{D}}\rho_{w}(x)-\log\left(L_{\theta^{*},\rho_{w}^{*}}^{\text{data}}({\cal D})(1+\varepsilon)-L_{\theta,\rho_{w}}^{\text{data}}({\cal D})\right)
\]

\subsection{Problem Formulation}

Let $\{(\x_n,\a_n,y_n)\}^N_{n=1}$ be a set of observations, where 
$\x_n$ is the information corresponding to individual $n$ (e.g., patient history), $\a_n$ is the intervention/action in one-hot vector encoding  (e.g., the selected treatment, which might be a single med or a combination of meds), and $y_n$ is the outcome (e.g., whether the treatment was successful or not). Our objective is to characterize the function $f_\theta: \xa \mapsto y$, where $\xa = [\x, \a ]$, in a way that it generalizes well in unseen scenarios.

In addition to the observed data, we also have a set of soft rules or guidelines capturing the intuition of experts in the field when choosing the intervention. Rules might reflect tolerability concerns, safety measures, or administrative requirements. Depending on each case, rules might be more or less correlated with the outcome of interest. We consider rules that either \textit{promote} or \textit{avoid} a given set of actions\footnote{\textit{Avoid} rules can be expressed as the complementary of \textit{promote} rules.}. Our objective is twofolds. First, by incorporating these rules into the data-driven model, we seek to guide the learning algorithm towards models that not only get a high fidelity score w.r.t the observed data, but also follow the rules as often as possible. Second, we want to unravel the existing correlation between the rules and the outcome to eventually improve outcome predictions.
%The hypothesis is that there is a global underlying function $g$ such that $y = g(\x,\a,\c)$.

Let $\left \{R_k: \xa \mapsto \big( A_k(\xa) \Rightarrow B_k(\xa) \big) \right\}^K_{k=1}$ be the set of implication function rules. The antecedent $A_k(\xa) = \mathbbm{1}[\x \in \mathcal{S}_k]$ refers to a constraint on the space $\mathcal{S}$ of patient states (e.g., overweight, insomnia, etc), while the consequent $B_k(\xa) = \mathbbm{1}[\a \in  \mathcal{A}_k]$ is a constraint on the space of interventions $\mathcal{A}$ (e.g., sedating drugs).\footnote{For the time being, we consider hard constraints in the antecendent and consequent, but these can be relaxed later on into soft conditions.} Let $c_k$ be the \textit{compliance} of rule $k$ (i.e., whether the rule was followed or not), corresponding to the realization of rule $R_k$ for input $\xa$. The compliance term $c_k$ can take three possible values:
\begin{eqnarray}
c_k = R_k(\xa) = \left\{ \begin{array}{ll}
+1.0 & \mbox{if $A_k(\xa) \wedge B_k(\xa)$}; \qquad \qquad \;\;\; \textrm{(rule followed)}\\
\; \; \;  0.0 & \mbox{if $A_k(\xa) \wedge \neg \, B_k(\xa)$};  \qquad \qquad \textrm{(rule not followed)}\\
-1.0 & \mbox{if $\neg A_k(\xa)$}. \qquad \qquad \qquad \qquad \quad \; \textrm{(rule not applicable)} \end{array} \right.
\end{eqnarray}\label{eq:compliance}

\paragraph{Loss Function.}
Let $\y \in \{0,1\}^{N \times 1}$ be the vector of outcomes, $\hat{y} \in [0,1]^{N \times 1}$ the predicted outcomes, and $\c \in \{0,1,-1\}^{N \times K}$ the compliance matrix for $N$ patients and $K$ rules.

\subsection{Inference}

\begin{enumerate}
	\item Unconstrained training
	\item Constrained training with warm initialization
\end{enumerate}
\begin{itemize}
	\item what are the effects of t and epsilon? both influence constraint satisfiability
	\item does this loss encourage improvements on performance in step 2? yes
\end{itemize}

Tricks to avoid local minima empirically
\begin{itemize}
	\item Important that $f_{w}(x)$ and $g(x)$ have the same scale
	\item Augment input features with higher-order polynomial terms
	\item Augment input features with local error rates for $f_{w}(x)$ and
	$g(x)$
	\item Alternate optimization (EM-schemes)
\end{itemize}

==> 04_experiments.tex <==
\section{Results}

\paragraph{Baselines}
\begin{itemize}
	\item Human-only always, and mean value for regions without rules
	\item Machine learning-only
	\item standard Mixture of Experts
	\item maybe Sontag paper?
	\item ours
\end{itemize}

We will consider two different operation regimes:

\begin{itemize}
	\item Alternative regime A: rules are not predictive, but capture other desiderata/benefits for the downstream application (safety, credibility, etc)
	\item Predictive regime B: rules are predictive (so should help improve accuracy as well). In practice, there is a continuous between these two regimes. In the generation of toy data, we control this balance between regimes with one hyperparameter.
\end{itemize}

\begin{itemize}
	\item Approach helps select a model that complies more with the rules while exhibiting ``good enough'' accuracy [table reporting accuracy and compliance in \%] (alternative regime A)
	
	\item In situations where expert rules are correlated with the outcome of interest, rules should help improve accuracy of the classifiers. Demonstrate with toy or semi-synthetic dataset. [table reporting accuracy and compliance in \%] (predictive regime B)
	
	\item We are able to obtain at least same accuracy with less data. (probably only in predictive regime B)
	
	\item We converge faster. (probably only in predictive regime B)
	
	\item Interpretability benefits
\end{itemize}
First three key advantages described in (Chattha et.al, 2019), useful resource to check types of plots.

\subsection*{Psychiatric dataset}

\subsection*{HIV}

==> 05_conclusion.tex <==
%\section*{Discussion}
%
% We aim to detect input-regions where rules can be followed.
% MEL: below, benefits on why ML systems that align with human rules are desirable, maybe good for discussion?
%Indeed, emitting recommendations that follow human intuitions has several advantages. a) benefits not captured by predictive performance: safety, tolerability, cost, etc. b) predictive performance: eventually, human rules might help improve performance (if guidelines aligned with outcome). c) credibility: a model that aligns with human knowledge when possible is easier to trust, inspect, and more likely to be deployed~\cite{wang_learning_2018}. d) Humans remain in charge (current status-quo, so interventions that suggest minimal (differential) changes will be easier to adopt + humans do not loose faculties or cognitive engagement).
%
%\begin{itemize}
%	\item under limited model capacity, benefits of having the data-based classifier not to focus on regions where humans perform well.
%	\item Even if we have unlimited model capacity, sample intensive to learn complex nonlinear decision boundaries.
%	\item Even if infinite data, expert might have additional side-information that allows to separate the data.
%\end{itemize}

%\begin{enumerate}
%	\item Re improving optimization of current MoE model: Two options available,
%	both lead to local optima, but might improve convergence (better local
%	optima):
%	\begin{enumerate}
%		\item alternating optimization (still prone to local optima) + warm initialization
%		\item minimize a convex majorizer (local convex approximation): this is
%		similar to David Sontag's group paper (NOPE)
%		\item explore whether global guarantees are possible (Gridlock paper) -
%		Javier
%	\end{enumerate}
%	\item How to flag OOD regions when both experts don't know (in psych data,
%	data so noisy, we might end up flagging everything, how to avoid?
%	penalty on number of flags)
%	\begin{enumerate}
%		\item for the time being, use an additional output variable to flag regions
%	\end{enumerate}
%	\item How to address the non-identifiability problem: simple gating function
%	and complicated experts VS complex gating function and simple experts?
%	\begin{itemize}
%		\item maximizing usage of human guidelines with unbounded capacity of the
%		gating function prone to overfitting
%		\item to alleviate this, added standard regularization to gating function
%		(tree with penalty on depth) 
%	\end{itemize}
%	\item (related to previous point) What are desirable gating function properties?
%	local vs global, better interpretability - we might need a way to
%	adjust complexity automatically - what makes a gating function easier
%	to interpret than another? (lower complexity? or input-axis aligned
%	regions)? (should the gating function be a tree?)
%	\item if both experts right, should data-based classifier ignore, or provide
%	complementary information if possible)? that is, differential explanation?
%	Two options: - If both agree, ignore data-based model (so same as
%	only having expert rule only) - if both agree, we should be able to
%	predict with more confidence, and eventually, provide complementary
%	explanation
%\end{enumerate}

\section{Conclusion}


==> additional_tables.tex <==
\begin{table}[h!]
	\centering
	\begin{tabular}{r|cc|ccc}\toprule
		\midrule
		Baselines & accuracy (\%) & AUC & soft coverage (\%) & hard coverage & ML agreement (\%) \\
		\midrule
		Human only & 49.87 & - & 100.0 & -\\
		\\
		No tuning of threshold \\
		MLonly & 64.12 $\pm$ 1.06 & 0.70 $\pm$ 0.01 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & - \\
		unconstrained & 63.47 $\pm$ 1.26 & 0.69 $\pm$ 0.01 & 30.93 $\pm$ 1.95 & 0.10 $\pm$ 0.20 & 46.36 $\pm$ 8.37 \\
		logBarrier & 63.91 $\pm$ 1.04 & 0.68 $\pm$ 0.02 & 48.64 $\pm$ 1.71 & 41.60 $\pm$ 10.73 & 14.01 $\pm$ 7.67 \\
		proj & 61.66 $\pm$ 3.10 & 0.64 $\pm$ 0.05 & 49.49 $\pm$ 5.90 & 36.62 $\pm$ 23.20 & 32.85 $\pm$ 9.99 \\
		\\
		Tuning based on AUC \\
		MLonly & 64.12 $\pm$ 1.06 & 0.70 $\pm$ 0.01 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & - \\
		unconstrained & 63.06 $\pm$ 1.66 & 0.69 $\pm$ 0.01 & 30.93 $\pm$ 1.95 & 3.50 $\pm$ 4.24 & 41.19 $\pm$ 9.99 \\
		logBarrier & 63.55 $\pm$ 1.10 & 0.69 $\pm$ 0.01 & 48.64 $\pm$ 1.71 & 18.34 $\pm$ 7.23 & 24.70 $\pm$ 7.17 \\
		proj & 63.81 $\pm$ 0.89 & 0.69 $\pm$ 0.01 & 49.49 $\pm$ 5.90 & 5.26 $\pm$ 6.54 & 45.87 $\pm$ 7.33 \\
		\\
		Tuning based on Accuracy \\
		MLonly & 63.86 $\pm$ 1.42 & 0.70 $\pm$ 0.01 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 43.68 $\pm$ 5.17 \\
		unconstrained & 64.40 $\pm$ 0.86 & 0.69 $\pm$ 0.01 & 30.93 $\pm$ 1.95 & 22.30 $\pm$ 12.59 & 31.26 $\pm$ 12.40 \\
		logBarrier & 64.59 $\pm$ 1.03 & 0.69 $\pm$ 0.02 & 48.64 $\pm$ 1.71 & 35.60 $\pm$ 10.81 & 17.57 $\pm$ 6.42 \\
		proj & 63.68 $\pm$ 1.41 & 0.67 $\pm$ 0.02 & 49.49 $\pm$ 5.90 & 24.17 $\pm$ 13.27 & 33.70 $\pm$ 11.50 \\
		\bottomrule
	\end{tabular}
	\caption{\label{tab:table1} \textbf{Performance vs Coverage (Psychiatry)}: Preferential MoE relies much more often on human expertise while preserving predictive performance. Predictive performance measured by Area-Under-the-operating-ROC-Curve (AUC) and percentage of correct predictions (accuracy) in the test set; Coverage refers to the percentage of predictions based on the human rules.}
\end{table}

\begin{table}[h!]
	\centering
	\begin{tabular}{r|cc|ccc}\toprule
		\midrule
		Baselines & accuracy (\%) & AUC & soft coverage (\%) & hard coverage & ML agreement (\%) \\
		\midrule
		Human only & 49.87 & - & 100.0 & -\\
		\\
		No tuning of threshold \\
		MLonly & 64.17 $\pm$ 0.79 & 0.70 $\pm$ 0.01 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 45.85 $\pm$ 2.81 \\
		unconstrained & 63.34 $\pm$ 1.48 & 0.69 $\pm$ 0.01 & 31.41 $\pm$ 2.40 & 0.21 $\pm$ 0.24 & 45.62 $\pm$ 9.85 \\
		logBarrier & 63.83 $\pm$ 1.43 & 0.68 $\pm$ 0.03 & 48.34 $\pm$ 2.29 & 39.98 $\pm$ 13.82 & 17.19 $\pm$ 8.97 \\
		proj & 64.30 $\pm$ 0.69 & 0.68 $\pm$ 0.01 & 45.06 $\pm$ 1.59 & 20.18 $\pm$ 7.23 & 39.10 $\pm$ 7.80 \\
		\\
		Tuning based on AUC \\
		MLonly & 64.17 $\pm$ 0.79 & 0.70 $\pm$ 0.01 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & nan $\pm$ nan \\
		unconstrained & 62.51 $\pm$ 1.99 & 0.69 $\pm$ 0.01 & 31.41 $\pm$ 2.40 & 5.31 $\pm$ 4.59 & 36.02 $\pm$ 9.48 \\
		logBarrier & 63.60 $\pm$ 1.11 & 0.70 $\pm$ 0.01 & 48.34 $\pm$ 2.29 & 16.65 $\pm$ 3.51 & 27.83 $\pm$ 6.44 \\
		proj & 64.04 $\pm$ 0.65 & 0.69 $\pm$ 0.01 & 45.06 $\pm$ 1.59 & 6.41 $\pm$ 3.95 & 46.08 $\pm$ 5.88 \\
		\\
		Tuning based on Accuracy \\
		MLonly & 63.68 $\pm$ 0.82 & 0.70 $\pm$ 0.01 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 43.65 $\pm$ 2.50 \\
		unconstrained & 65.00 $\pm$ 0.45 & 0.69 $\pm$ 0.01 & 31.41 $\pm$ 2.40 & 25.98 $\pm$ 13.64 & 25.52 $\pm$ 13.44 \\
		logBarrier & 64.66 $\pm$ 1.07 & 0.69 $\pm$ 0.02 & 48.34 $\pm$ 2.29 & 42.22 $\pm$ 6.65 & 14.40 $\pm$ 4.29 \\
		proj & 64.69 $\pm$ 0.41 & 0.68 $\pm$ 0.01 & 45.06 $\pm$ 1.59 & 35.55 $\pm$ 7.01 & 26.14 $\pm$ 7.63 \\
		\\
		L1=0.1\\
		MLonly & 64.17 $\pm$ 0.79 & 0.70 $\pm$ 0.01 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 45.85 $\pm$ 2.81 \\
		unconstrained & 63.42 $\pm$ 1.35 & 0.69 $\pm$ 0.01 & 37.84 $\pm$ 1.67 & 0.00 $\pm$ 0.00 & 42.72 $\pm$ 4.65 \\
		logBarrier & 60.70 $\pm$ 1.80 & 0.62 $\pm$ 0.04 & 48.86 $\pm$ 4.46 & 45.06 $\pm$ 22.66 & 27.96 $\pm$ 10.40 \\
		proj & 58.91 $\pm$ 1.36 & 0.59 $\pm$ 0.02 & 51.68 $\pm$ 0.91 & 57.04 $\pm$ 6.64 & 40.51 $\pm$ 9.31 \\
		\\
		MLonly & 64.17 $\pm$ 0.79 & 0.70 $\pm$ 0.01 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & nan $\pm$ nan \\
		unconstrained & 63.42 $\pm$ 1.35 & 0.69 $\pm$ 0.01 & 37.84 $\pm$ 1.67 & 0.00 $\pm$ 0.00 & 42.72 $\pm$ 4.65 \\
		logBarrier & 62.49 $\pm$ 1.15 & 0.68 $\pm$ 0.01 & 48.86 $\pm$ 4.46 & 6.82 $\pm$ 6.02 & 34.95 $\pm$ 9.79 \\
		proj & 63.11 $\pm$ 1.13 & 0.68 $\pm$ 0.01 & 51.68 $\pm$ 0.91 & 2.21 $\pm$ 1.50 & 44.79 $\pm$ 9.28 \\
		\\
		MLonly & 63.68 $\pm$ 0.82 & 0.70 $\pm$ 0.01 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 43.65 $\pm$ 2.50 \\
		unconstrained & 64.02 $\pm$ 0.99 & 0.69 $\pm$ 0.02 & 37.84 $\pm$ 1.67 & 6.59 $\pm$ 11.53 & 35.07 $\pm$ 12.56 \\
		logBarrier & 62.85 $\pm$ 0.95 & 0.67 $\pm$ 0.02 & 48.86 $\pm$ 4.46 & 16.65 $\pm$ 11.87 & 33.80 $\pm$ 8.08 \\
		proj & 61.74 $\pm$ 2.06 & 0.64 $\pm$ 0.04 & 51.68 $\pm$ 0.91 & 23.70 $\pm$ 19.37 & 39.41 $\pm$ 4.46 \\
		\bottomrule
	\end{tabular}
	\caption{\label{tab:table1} \textbf{Performance vs Coverage (Psychiatry)}: \textbf{L1=0.05, 5 seeds} Preferential MoE relies much more often on human expertise while preserving predictive performance. Predictive performance measured by Area-Under-the-operating-ROC-Curve (AUC) and percentage of correct predictions (accuracy) in the test set; Coverage refers to the percentage of predictions based on the human rules.}
\end{table}

\begin{table}[h!]
	\centering
	\begin{tabular}{r|cc|ccc}\toprule
		\midrule
		Baselines & accuracy (\%) & AUC & soft coverage (\%) & hard coverage & ML agreement (\%) \\
		\midrule
		Human only & 49.87 & - & 100.0 & -\\
		\\
		No tuning of threshold \\
		MLonly & 64.12 $\pm$ 1.06 & 0.70 $\pm$ 0.01 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & 45.13 $\pm$ 4.69 \\
		unconstrained & 63.15 $\pm$ 1.13 & 0.69 $\pm$ 0.01 & 38.58 $\pm$ 1.64 & 0.00 $\pm$ 0.00 & 41.18 $\pm$ 6.25 \\
		logBarrier & 60.31 $\pm$ 2.23 & 0.61 $\pm$ 0.04 & 50.19 $\pm$ 3.62 & 53.13 $\pm$ 22.26 & 22.22 $\pm$ 10.93 \\
		proj & 56.33 $\pm$ 3.07 & 0.56 $\pm$ 0.03 & 55.69 $\pm$ 5.19 & 67.93 $\pm$ 16.59 & 32.18 $\pm$ 12.47 \\
		\\
		Tuning based on AUC \\
		MLonly & 64.12 $\pm$ 1.06 & 0.70 $\pm$ 0.01 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & - \\
		unconstrained & 63.15 $\pm$ 1.13 & 0.69 $\pm$ 0.01 & 38.58 $\pm$ 1.64 & 0.00 $\pm$ 0.00 & - \\
		logBarrier & 62.84 $\pm$ 1.08 & 0.68 $\pm$ 0.01 & 50.19 $\pm$ 3.62 & 9.48 $\pm$ 7.18 & 34.52 $\pm$ 10.68 \\
		proj & 62.95 $\pm$ 0.97 & 0.69 $\pm$ 0.01 & 55.69 $\pm$ 5.19 & 1.12 $\pm$ 1.52 & 41.80 $\pm$ 8.82 \\
		\\
		Tuning based on Accuracy \\
		MLonly & 63.86 $\pm$ 1.42 & 0.70 $\pm$ 0.01 & 0.00 $\pm$ 0.00 & 0.00 $\pm$ 0.00 & - \\
		unconstrained & 63.37 $\pm$ 0.99 & 0.69 $\pm$ 0.02 & 38.58 $\pm$ 1.64 & 9.45 $\pm$ 11.13 & 35.41 $\pm$ 10.70 \\
		logBarrier & 62.23 $\pm$ 1.91 & 0.66 $\pm$ 0.03 & 50.19 $\pm$ 3.62 & 22.54 $\pm$ 12.47 & 28.86 $\pm$ 8.28 \\
		proj & 61.19 $\pm$ 1.69 & 0.64 $\pm$ 0.03 & 55.69 $\pm$ 5.19 & 18.12 $\pm$ 15.10 & 38.94 $\pm$ 4.23 \\
		\bottomrule
	\end{tabular}
	\caption{\label{tab:table1} \textbf{Performance vs Coverage (Psychiatry)}: \textbf{L1=0.1} Preferential MoE relies much more often on human expertise while preserving predictive performance. Predictive performance measured by Area-Under-the-operating-ROC-Curve (AUC) and percentage of correct predictions (accuracy) in the test set; Coverage refers to the percentage of predictions based on the human rules.}
\end{table}

\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{./figs/hist_rhos.png}
	\caption{\textbf{Histograms for $\boldsymbol{\rho(x)}$ in the test set.} Preferential MoE pushes up the values for the gating functions, favoring relying on human decision rules in certain regions of the input space.}
	\label{fig:histrhos-thtypeauc-l10}
\end{figure}

%\begin{table}[h!]
%	\centering
%	\begin{tabular}{c|cccc}\toprule
%		\midrule
%		& \multicolumn{2}{c}{AUC} & \multicolumn{2}{c}{soft coverage (\%)} \\
%		\multicolumn{1}{c|}{Baselines} & mean & CI & mean & CI \\
%		\midrule
%		ML only & 0.70 & [0.69-0.71] & 0.00 & [0.00-0.00] \\
%		standard MoE (unconstrained) & 0.70 & [0.70-0.71] & 37.84 & [35.79-39.99] \\
%		Preferential MoE (log barrier) & 0.70 & [0.70-0.70] & 48.86 & [42.13-51.36] \\
%		Preferential MoE (projected gradient) & 0.70 & [0.70-0.71] & 51.68 & [50.69-52.83] \\
%		\bottomrule
%	\end{tabular}
%	\caption{\label{tab:table1} \textbf{Performance vs Coverage (Psychiatry)}: \textbf{L1=0.1} Preferential MoE relies much more often on human expertise while preserving predictive performance. Predictive performance measured by Area-Under-the-operating-ROC-Curve (AUC) and percentage of correct predictions (accuracy) in the test set; Coverage refers to the percentage of predictions based on the human rules.}
%\end{table}
